A Weighted Quiver Kernel using Functor Homology

In this paper, we propose a new homological method to study weighted directed networks. Our model of such networks is a directed graph $Q$ equipped with a weight function $w$ on the set $Q_{1}$ of arrows in $Q$. We require that the range $W$ of our weight function is equipped with an addition or a multiplication, i.e., $W$ is a monoid in the mathematical terminology. When $W$ is equipped with a representation on a vector space $M$, the standard method of homological algebra allows us to define the homology groups $H_{*}(Q,w;M)$. It is known that when $Q$ has no oriented cycles, $H_{n}(Q,w;M)=0$ for $n\ge 2$ and $H_{1}(Q,w;M)$ can be easily computed. This fact allows us to define a new graph kernel for weighted directed graphs. We made two sample computations with real data and found that our method is practically applicable.

==> functor_homology_functoriality.tex <==
\subsection{Functoriality}
\label{functor_homology_functoriality}

\begin{definition}
 Let $\Cat\downarrow\lMod{k}$ be the category whose objects are functors
 $F:C\to\lMod{k}$ for a small category $C$. 
 A morphism from $F: C\to \lMod{k}$ to $G: D\to \lMod{k}$ is a pair
 $\bm{\varphi}=(\underline{\varphi},\varphi)$ of a functor
 $\underline{\varphi}:C\to D$ and a natural transformation
 $\varphi : F \to G\circ \varphi$. 
\end{definition}

Let us show that our homology is a functor on this category.

\begin{lemma}
 For a morphism $\bm{\varphi}=(\underline{\varphi},\varphi): F \to G$
 define 
 \[
  \bm{\varphi}_{n} : B_{n}(C;F) \rarrow{} B_{n}(D;G)
 \]
 by
 \[
  \bm{\varphi}_{n}((u_{n},\ldots,u_{1})\otimes m) =
 (\underline{\varphi}(u_{n}),\ldots, 
 \underline{\varphi}(u_{1}))\otimes \varphi(s(u_{1}))(m).
 \]
 Then the collection $\bm{\varphi}_{*}=\{\bm{\varphi}_{n}\}$ forms a map
 of simplicial modules. 

 Thus we obtain a functor
 \[
  H_{n} : \Cat \downarrow\lMod{k} \rarrow{} \lMod{k}.
 \]
\end{lemma}

\begin{example}
 \label{example:functoriality_of_homology_of_weighted_quivers}
 Consider the situation in Proposition
 \ref{induced_map_for_homology_of_weighted_quivers}. 
 We  have weighted quivers $w:Q\to W$ and $w':Q'\to W'$ 
 and a morphism of weighted quivers $f:(Q,w)\to (Q',w')$.
 We also have morphisms of representations 
 $(f_{w},\varphi): (W,M)\to (W',M')$.

 The weighted quivers generate free weighted categories
 $(F(Q),\tilde{w})$ and $(F(Q'),\tilde{w'})$.
 The map $f$ induces a functor $F(f): F(Q)\to F(Q')$ on the free
 categories. 

 Under the identifications in Example
 \ref{example:representation_as_functor}, we regard actions of $W$ and
 $W'$ on $M$ and $M'$ as functors
 $\mu_{M}:W\to \lMod{k}$ and $\mu_{M'}:W'\to \lMod{k}$.
 Then $\varphi$ can be regarded as a natural transformation
 $\varphi: \mu_{M}\Rightarrow \mu_{M'}$.
 
 And we obtain a morphism $(f,\varphi)$ from $\mu_{M}\circ \tilde{w}$ to
 $\mu_{M'}\circ \tilde{w'}$. 
 The map induced from this morphism is essentially the map in
 Proposition \ref{induced_map_for_homology_of_weighted_quivers}.
\end{example}


==> functor_homology_homotopy_invariance.tex <==
\subsection{Homotopy Invariance}
\label{functor_homology_homotopy_invariance}

The category $\Cat\downarrow\lMod{k}$ has a structure of
$2$-category. Let us show that $2$-morphisms induce simplicial
homotopies on $B_{*}(-)$. 

\begin{definition}
 Let $F:C\to \lMod{k}$ and $G:D\to\lMod{k}$ be functors.
 For morphisms $\bm{\varphi}$ and $\bm{\psi}$ from $F$ to $G$, a
 \emph{$2$-morphism} from $\bm{\varphi}$  to $\bm{\psi}$ is a natural
 transformation $\theta:\underline{\varphi}\to\underline{\psi}$
 satisfying $\psi=\theta\circ\varphi$.
\end{definition}

\begin{proposition}
 \label{homotopy_invariance_of_functor_homology}
 Let $F:C\to \lMod{k}$ and $G:D\to\lMod{k}$ be functors
 and $\bm{\varphi}$ and $\bm{\psi}$ morphisms from $F$ to $G$.
 Then a $2$-morphism $\theta$ from $\bm{\varphi}$ to $\bm{\psi}$
 induces a simplcial homotopy from $\bm{\varphi}_{*}$ to
 $\bm{\psi}_{*}$.

 Hence the induced maps on functor homologies are identical
 \[
 H(\bm{\varphi}) = H(\bm{\psi}) : H_{*}(C;F) \rarrow{} H_{*}(D;G).
 \]
\end{proposition}

\begin{proof}
 For a $2$-morphism $\theta$ from $\bm{\varphi}$ to $\bm{\psi}$, we
 define a simplicial map
 \[
  \bm{\theta}_{*} : B_{*}(C,F)\times\Delta^{1} \rarrow{} B_{*}(D,G)
 \]
 as follows.

 We use the identification $\Delta^{1}=N([1])$. The natural
 transformation $\theta:\underline{\varphi}\to\underline{\psi}$ can be
 regarded as a functor $\underline{\theta} : C\times [1] \to D$ in the
 usual way.
 Consider the two functors
 \[
 F\circ\pr_{1},G\circ\underline{\theta} : C\times[1] \rarrow{}
 \lMod{k}. 
 \]
 Define a natural transformation
 \[
 \theta : F\circ\pr_{1} \Longrightarrow{} G\circ\underline{\theta}
 \]
 by
 \begin{align*}
  \theta(x,0) & = \varphi(x) : F(x) \rarrow{}
  (D\circ\underline{\varphi})(x) \\
  \theta(x,1) & = \psi(x): F(x) \rarrow{} (D\circ\underline{\psi})(x)
 \end{align*}
 on objects. The condition $\psi=\theta\circ\varphi$ guarantees that
 this is a natural transformation.
 Thus we obtain a morphism
 \[
  \bm{\theta}=(\underline{\theta},\theta):(C\times[1],F\circ\pr_{1})
 \rarrow{} (D,G) 
 \]
 in $\Cat\downarrow\lMod{k}$.
 Under the identification
 \[
  B_{*}(C\times [1];F\circ \pr_{1}) \cong B_{*}(C;F)\times N([1]) =
 B_{*}(C;F)\times\Delta^{1}, 
 \]
 The morphism $\bm{\theta}$ induces a simplicial map
 \[
  \bm{\theta}_{*}: B_{*}(C;F)\times\Delta^{1} \rarrow{} B_{*}(D;G),
 \]
 which is a simplicial homotopy from $\bm{\varphi}$ to $\bm{\psi}$.
\end{proof}

\begin{corollary}
 Let $F:C\to\lMod{k}$ and $G:D\to\lMod{k}$ be functors.
 If there exist morphisms $\bm{\varphi}: (C,F)\to (D,G)$ and
 $\bm{\psi}: (D,G)\to (C,F)$ and $2$-morphisms
 $\theta:\bm{\varphi}\Rightarrow\bm{\psi}$ and
 $\xi:\bm{\psi}\Rightarrow\bm{\varphi}$, then $\bm{\varphi}$ induces an
 isomorphism
 $\bm{\psi}_{*} : H_{*}(C;F)\rarrow{}H_{*}(D,G)$ 
 whose inverse is given by $\bm{\psi}_{*}$. 
\end{corollary}

\begin{example}
 \label{example:homotopy_invariance_of_homology_of_weighted_quivers}
 Consider the situation in Proposition
 \ref{homotopy_invariance_of_homology_of_weighted_quivers}. 
 We have morphisms $f,g: (Q,w)\to (Q',w')$ of weighted quivers,
 morphisms $\varphi,\psi:(W,M)\to (W',M')$ of representations, and a
 transformation $\theta$ from $(f,\varphi)$ to $(g,\psi)$. 

 As we have seen in Example
 \ref{example:functoriality_of_homology_of_weighted_quivers}, 
 we have morphis
 $(f,\varphi)$ and $(g,\psi)$ from
 $\mu_{M}\circ \tilde{w}$ to $\mu_{M'}\circ\tilde{w'}$ in
 $\Cat\downarrow\lMod{k}$.  

 The requirement on $\theta$ to be a transformation from $(f,\varphi)$
 to $(g,\psi)$ guarantees that $\theta$ induces a $2$-morphism 
 from $(f,\varphi)$ to $(g,\varphi)$.
 This proves Proposition
 \ref{homotopy_invariance_of_homology_of_weighted_quivers} as a
 corollary to Proposition 
 \ref{homotopy_invariance_of_functor_homology}. 
\end{example}

==> homology_of_weighted_category_functoriality.tex <==
\subsection{The Functoriality of Homology of Weighted Categories}
\label{homology_of_weighted_category_functoriality}

One of the most important properties of homology groups is the
functoriality. In fact, categories, functors, and natural
transformations were introduced by Eilenberg and Mac\,Lane in roder to
describe properties of homology groups.

The functoriality of homology groups is useful when we compare homology
groups of two objects. We first need to introduce morphisms of weighted
quivers.

\begin{definition}
 Let $w:Q\to W$ and $w':Q'\to W'$ be weighted quivers. A \emph{morphism of
 weighted quivers} from $(Q,w)$ to $(Q',w')$ is a triple
 $f=(f_{0},f_{1},f_{w})$ of maps
 \begin{align*}
  f_{0} & : Q_{0} \rarrow{} Q'_{0} \\
  f_{1} & : Q_{1} \rarrow{} Q'_{1} \\
  f_{w} & : W \rarrow{} W'
 \end{align*}
 satisfying the following conditions:
 \begin{enumerate}
  \item $f$ preserves the source, i.e.~$f_{0}\circ s = s\circ f_{1}$.
  \item $f$ preserves the target, i.e.~$f_{0}\circ t = t\circ f_{1}$.
  \item $f_{1}$ and $f_{w}$ are compatible in the sense that
	$w'\circ f_{1} = f_{w}\circ w$.
 \end{enumerate}
\end{definition}

We also need morphisms between coefficients.

\begin{definition}
 Suppose monoids $W$ and $W'$ act on $k$-modules $M$ and $M'$ from the
 left, respectively. A \emph{morphism of representations} from $(W,M)$
 to $(W',M')$ is a pair $(f,\varphi)$ of a homorophism of monoids
 $f: W\to W'$ and a $k$-homomorphism $\varphi: M\to M'$ such that the
 following diagram is commutative
 \[
  \begin{diagram}
   \node{W\times M} \arrow{s,l}{f\times\varphi} \arrow{e} \node{M}
   \arrow{s,r}{\varphi} \\ 
   \node{W'\times M'} \arrow{e} \node{M'.}
  \end{diagram}
 \]
\end{definition}

Now we are ready to state the functoriality of our homology.

\begin{proposition}
 \label{induced_map_for_homology_of_weighted_quivers}
 Suppose we are given a morphism $f:(Q,w)\to (Q',w')$ of weighted
 acyclic quivers. Suppose further that we have a morphism of
 representations $(f_{w},\varphi):(W,M)\to (W',M')$. 
 Then we have an induced map
 \[
  (f,\varphi)_{*} : H_{n}(Q,w;M) \rarrow{} H_{n}(Q',w',M').
 \]

 More generally, a morphism $f:(C,w)\to (C',w')$ of weighted acyclic
 categories and a morphism $(f_{w},\varphi):(W,M)\to (W',M')$ induce a
 map
 \[
  (f,\varphi)_{*} : H_{n}(C,w;M) \rarrow{} H_{n}(C',w',M').
 \]
\end{proposition}

\begin{proof}
 This is a consequence of the functoriality of more general homology
 stated in \S\ref{functor_homology_functoriality}.
 However, for the convenience of the reader, we give a direct
 construction of $(f,\varphi)_{*}$ for acyclic quivers.

 In order to obtain a map between homology groups, tt suffices to define
 a chain map
 \[
 \barC_{n}(f,\varphi) : \barC_{n}(F(Q);M) \rarrow{}
 \barC_{n}(F(Q');M'). 
 \]
 It is defined by
 \[
  \barC_{n}(f,\varphi)((u_{n},\ldots,u_{1})\otimes m) =
 (F(f)_{1}(u_{n}), 
 \ldots, F(f)_{1}(u_{1}))\otimes \varphi(m),
 \]
 where $F(f): F(Q)\to F(Q')$ is the functor induced from $f$.
 It is left to the reader to verify that these maps define a chain map
 \[
 \barC_{*}(f,\varphi) : \barC_{*}(F(Q);M) \rarrow{}
 \barC_{*}(F(Q');M'). 
 \]
 The above argument works without a change to weighted small categories.
\end{proof}

\begin{remark}
 See Example \ref{example:functoriality_of_homology_of_weighted_quivers}
 for details.
\end{remark}

\begin{example}
 
\end{example}

==> homology_of_weighted_category_homotopy_invariance.tex <==
\subsection{The Homotopy Invariance of Homology of Weighted Categories}
\label{homology_of_weighted_category_homotopy_invariance}

In order to state the homotopy invariance, we need to introduce
transformations of morphisms of weighted categories.

\begin{definition}
 Let $f: (C,w)\to (D,w')$ be a morphism of weighted categories and
 $\varphi:(W,M)\to (W',M')$ be a morphism of representations.
 Given another morphism $g:(C,w)\to (D,w')$ of weighted categories and a
 morphism $\psi:(W,M)\to (W',M')$, 

 A \emph{transformation} from $(f,\varphi)$ to $(g,\psi)$ is a 
 natural transformations 
 $\theta : (f_{0},f_{1}) \Rightarrow (g_{0},g_{1})$ 
 making the following diagram commutative for all $x\in C_{0}$
 \[
  \begin{diagram}
   \node{M}
   \arrow{s,l}{\psi} 
   \arrow{e,t}{\varphi} \node{M'} \arrow{e,=}
   \node{\mu_{M'}\circ\tilde{w'}\circ f(x)} \arrow{s,r}{\mu_{M'}\circ
   \tilde{w'}\circ \theta(x)} \\
   \node{M'} \arrow[2]{e,=} \node{}  \node{\mu_{M'}\circ\tilde{w'}\circ g(x)}
  \end{diagram}
 \]
\end{definition}

\begin{proposition}
 \label{homotopy_invariance_of_homology_of_weighted_quivers}
 Let $f,g: (Q,w)\to (Q',w')$ be morphisms of weighted acyclic quivers
 and $\varphi,\psi:(W,M)\to (W',M')$ be morphisms of representations.
 Then any transformation $\theta$ from $(f,\varphi)$ to $(g,\psi)$
 induces a chain homotopy from $\barC_{*}(f,\varphi)$ to
 $\barC_{*}(g,\psi)$. 
 
 Hence if such a transformation exists, the induced maps coincide
 \[
 (f,\varphi)_{*} = (g,\psi)_{*} : H_{n}(Q,w;M) \rarrow{}
 H_{n}(Q',w';M'). 
 \]
\end{proposition}

It is not easy to prove this fact. A proof is given as a corollary to a
general property of functor homologies in
\S\ref{functor_homology_homotopy_invariance}. See Example
\ref{example:homotopy_invariance_of_homology_of_weighted_quivers} for
details. 

==> homology_of_weighted_network.tex <==
\section{Homology of Weighted Directed Networks}
\label{homology_of_weighted_network}

Throughout this section, we fix a commutative ring $k$. When necessary,
we assume that $k$ is a field.
 
\input{small_category}
\input{homology_of_weighted_category}
%\input{standard_resolution}

%\input{homology_of_weighted_category_functoriality}
%\input{homology_of_weighted_category_homotopy_invariance}
%\input{length_filtration}


==> length_filtration.tex <==
\subsection{The Length Filtration}
\label{length_filtration}

In this section, we introduce the length filtration on the chain complex
$\barC_{*}(F(Q);M)$. 

\begin{definition}
 For a quiver $Q$ and a nonnegative integer, define
 a quiver $F^{\ell}(Q)$ by
 $F^{\ell}(Q)_{0}=Q_{0}$ and  
 \[
 F^{\ell}(Q)_{1} = \coprod_{n=0}^{\ell} N_{n}(Q).
 \]
 This is called the \emph{$\ell$-th power} of $Q$.

 The quiver $F^{\ell}(Q)$ is a subquiver of $F(Q)$. 
 When $Q$ has a weight $w$ with values in a monoid $W$, we have a weight
 $\tilde{w}$ on $F(Q)$. The restriction of $\tilde{w}$ to $F^{\ell}(Q)$
 is denoted by $w_{\ell}$.
\end{definition}

For $\ell<\infty$, $F^{\ell}(Q)$ is not a small
category. However, we may define a chain complex out of
$F^{\ell}(Q)$. 

\begin{definition}
 For a quiver $Q$ and a nonnegative integer $\ell$, the
 set of pairs of composable morphisms whose compositions belong to
 $F^{\ell}(Q)$ is denoted by $N_2^{\ell}(Q)$
 \[
 N_2^{\ell}(Q) = \set{(\gamma_{2},\gamma_{1}) \in
 N_{2}(F(Q))}{ \gamma_{2}\circ\gamma_{1}\in F^{\ell}(Q)} .
 \]
 More generally, define
 \[
 N^{\ell}_{n}(Q) =
 \set{(\gamma_{n},\ldots,\gamma_{1}) \in
 N_{n}(F(Q))}{\gamma_{n}\circ \cdots\circ \gamma_{1}\in
 F^{\ell}(Q)}.
 \]
 The collection $N^{\ell}(Q)=\{N_{n}^{\ell}(Q)\}_{n\ge 0}$ is
 called the \emph{$\ell$-truncated nerve} of $Q$.
\end{definition}

%\begin{remark}
% We have the following
% pullback diagram 
% \[
%  \begin{diagram}
%   \node{N_2^{\ell}(\Gamma)} \arrow{s} \arrow{e}
%   \node{F^{\ell}(\Gamma)_{1}} \arrow{s,J} \\ 
%   \node{N_{2}(F(\Gamma))} \arrow{e,b}{\circ}
%   \node{F(\Gamma)_{1}}. 
%  \end{diagram}
% \]
%\end{remark}

As we have done in \S\ref{small_category}, we remove identity morphisms
under the acyclicity assumption.

\begin{definition}
 For an acyclic quiver $Q$, define
 \[
 \overline{N}^{\ell}_{n}(Q) = \set{(\gamma_{n},\ldots,
 \gamma_{1}) \in N^{\ell}_{n}(Q)}{ \text{ None of }\gamma_{i}
 \text{ is the identity morphism.} }.
 \]
 The collection
 $\overline{N}^{\ell}(Q)=\{\overline{N}^{\ell}_{n}(Q)\}$ is
 called the \emph{$\ell$-truncated nondegenerate nerve of $Q$}.
\end{definition}

\begin{remark}
 $F^{\ell}(Q)$ has a structure of a ``partial category'' in the sense
 that compositions of morphisms are partially defined. This structure
 has been discovered by many people independently and named
 differently. For example, Bessis \cite{math/0610778} calls such a
 structure a \emph{germ}, R.~Milner \cite{Milner2006} calls it a
 \emph{precategory},  
 and Andersen and Kashaev \cite{1109.6295} call it a \emph{categroid}.
\end{remark}

\begin{definition}
 For an acyclic quiver $Q$ and a nonnegative integer $\ell$, the submodule of
 $\barC_{n}(F(Q);k)$ generated by $N_{n}^{\ell}(Q)$ is denoted by
 $\barC_{n}^{\ell}(Q;k)$. When $Q$ has a weight $w:F(Q)_{1}\to W$ and
 $W$ has a representation $M$, we define
 \[
  \barC_{n}^{\ell}(Q;M) = \barC_{n}^{\ell}(Q;k)\otimes M.
 \]
 It is straightforward to verify that the boundary homomorphisms on
 $\barC_{*}(F(Q);M)$ can be restricted to
 \[
  \partial^{\ell}_{n} : \barC_{n}^{\ell}(Q;M) \rarrow{}
 \barC_{n-1}^{\ell}(Q;M) 
 \]
 and defines a chain complex $\barC_{*}^{\ell}(Q;M)$. 
 The homology of this chain complex is denoted by $H^{\ell}_{*}(Q,w;M)$.
\end{definition}


